ScoRe-Flow: Complete Distributional Control via Score-Based Reinforcement Learning for Flow Matching

Flow Matching (FM) policies have emerged as an efficient backbone for robotic control, offering fast and expressive action generation that underpins recent large-scale embodied AI systems. However, FM policies trained via imitation learning inherit the limitations of demonstration data; surpassing suboptimal behaviors requires reinforcement learning (RL) fine-tuning. Recent methods convert deterministic flows into stochastic differential equations (SDEs) with learnable noise injection, enabling exploration and tractable likelihoods, but such noise-only control can compromise training efficiency when demonstrations already provide strong priors. We observe that modulating the drift via the score function, i.e., the gradient of log-density, steers exploration toward high-probability regions, improving stability. The score admits a closed-form expression from the velocity field, requiring no auxiliary networks. Based on this, we propose ScoRe-Flow, a score-based RL fine-tuning method that combines drift modulation with learned variance prediction to achieve decoupled control over the mean and variance of stochastic transitions. Experiments demonstrate that ScoRe-Flow achieves 2.4x faster convergence than flow-based SOTA on D4RL locomotion tasks and up to 5.4% higher success rates on Robomimic and Franka Kitchen manipulation tasks.

==> tables/main_results.tex <==
\begin{table*}[t]
\centering
\caption{Performance comparison across all benchmarks. We report final performance (mean $\pm$ std over 3 seeds) and wall-clock time to reach 90\% of final performance (in hours). For D4RL we report episode reward, for Robomimic we report success rate (\%), for Kitchen we report average tasks completed (out of 4). \textbf{Bold}: best, \underline{underline}: second best.}
\label{tab:main_results}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c|}{DPPO} & \multicolumn{2}{c|}{ReinFlow-R} & \multicolumn{2}{c|}{ReinFlow-S} & \multicolumn{2}{c|}{Score-SDE} & \multicolumn{2}{c}{\textbf{ScoRe-Flow (Ours)}} \\
Task & Perf. & Time & Perf. & Time & Perf. & Time & Perf. & Time & Perf. & Time \\
\midrule
\multicolumn{11}{l}{\textit{D4RL Locomotion (Episode Reward $\uparrow$, Time in hours $\downarrow$)}} \\
\midrule
Hopper-v2 & \textbf{3275$\pm$20} & 11.28 & 3204$\pm$36 & 1.10 & \underline{3253$\pm$24} & 0.60 & 3118$\pm$87 & \textbf{0.12} & 3233$\pm$39 & \underline{0.28} \\
Walker2d-v2 & 3896$\pm$62 & 0.66 & 4092$\pm$11 & 0.15 & \textbf{4202$\pm$26} & 0.11 & 3900$\pm$57 & \textbf{0.04} & \underline{4172$\pm$154} & \underline{0.10} \\
Ant-v2 & 3951$\pm$24 & 0.66 & 4021$\pm$25 & 0.32 & \textbf{4119$\pm$44} & 0.39 & 3980$\pm$29 & \underline{0.10} & \underline{4088$\pm$95} & \textbf{0.02} \\
Humanoid-v3 & 5001$\pm$20 & 1.32 & \underline{5041$\pm$6} & \underline{0.40} & 4801$\pm$134 & 0.42 & 4896$\pm$91 & 0.49 & \textbf{5100$\pm$47} & \textbf{0.23} \\
\midrule
\multicolumn{11}{l}{\textit{Robomimic (Success Rate \% $\uparrow$, Time in hours $\downarrow$)}} \\
\midrule
PickPlaceCan & 96.5$\pm$0.2 & 1.14 & 95.6$\pm$0.1 & 1.21 & 91.7$\pm$0.5 & 1.62 & \underline{96.8$\pm$0.2} & \underline{1.21} & \textbf{98.3$\pm$0.5} & \textbf{1.21} \\
Square & 73.5$\pm$4.2 & 16.66 & 71.5$\pm$2.7 & 11.63 & 71.4$\pm$2.1 & \underline{10.59} & \underline{74.3$\pm$1.3} & \textbf{11.05} & \textbf{79.9$\pm$0.6} & 12.42 \\
\midrule
\multicolumn{11}{l}{\textit{Franka Kitchen (Tasks Completed /4 $\uparrow$, Time in hours $\downarrow$)}} \\
\midrule
Complete & 3.8$\pm$0.1 & 1.15 & N/A & N/A & 3.9$\pm$0.0 & \underline{0.09} & \textbf{4.0$\pm$0.0} & 0.10 & \textbf{4.0$\pm$0.0} & \textbf{0.09} \\
Mixed & \textbf{3.4$\pm$0.5} & 1.15 & N/A & N/A & 3.0$\pm$0.0 & 0.15 & 3.0$\pm$0.0 & \textbf{0.11} & 3.0$\pm$0.0 & \textbf{0.11} \\
Partial & 3.3$\pm$0.4 & 2.54 & N/A & N/A & \underline{3.4$\pm$0.5} & \textbf{0.38} & 2.8$\pm$0.2 & \underline{0.64} & \textbf{3.8$\pm$0.2} & 1.45 \\
\bottomrule
\end{tabular}
\end{table*}

